Neuroplastic graph attention networks for nuclei segmentation in histopathology images

Modern histopathological image analysis relies on the segmentation of cell structures to derive quantitative metrics required in biomedical research and clinical diagnostics. State-of-the-art deep learning approaches predominantly apply convolutional layers in segmentation and are typically highly customized for a specific experimental configuration; often unable to generalize to unknown data. As the model capacity of classical convolutional layers is limited by a finite set of learned kernels, our approach uses a graph representation of the image and focuses on the node transitions in multiple magnifications. We propose a novel architecture for semantic segmentation of cell nuclei robust to differences in experimental configuration such as staining and variation of cell types. The architecture is comprised of a novel neuroplastic graph attention network based on residual graph attention layers and concurrent optimization of the graph structure representing multiple magnification levels of the histopathological image. The modification of graph structure, which generates the node features by projection, is as important to the architecture as the graph neural network itself. It determines the possible message flow and critical properties to optimize attention, graph structure, and node updates in a balanced magnification loss. In experimental evaluation, our framework outperforms ensembles of state-of-the-art neural networks, with a fraction of the neurons typically required, and sets new standards for the segmentation of new nuclei datasets.

==> oldMaterial <==
\begin{table*} 
    \centering 
    \begin{tabular}{l c c c c c c c c c} 
    & \multicolumn{2}{c}{\textbf{Dice-Coefficient}}& \multicolumn{2}{c}{\textbf{Jaccard Index (IoU)}} & \multicolumn{2}{c}{\textbf{Node Accuracy}}\\ 
    \cmidrule(l){2-3} 
    \cmidrule(l){4-5} 
    \cmidrule(l){6-7}     
    \textbf{Approach} & value & $\sigma$ & value & $\sigma$ & value & $\sigma$ \\ 
    \midrule   
    \textbf{final} & 0.843 & 0.021 & 0.856 & 0.029 & 0.810 & 0.026 \\           
    \bottomrule 
    \end{tabular}
    \caption{Experimental evaluation of semantic segmentation with various constellations. The metrics are calculated based on node-wise intersection with annotated ground truth. Metrics include Dice-Coefficient (F1 Score) and Jaccard Index (IOU) as well as the Pixel Accuracy. 
    } 
    \label{tab:segmentation} 
    \end{table*}
